Glacier Calving Front Segmentation Using Attention U-Net

An essential climate variable to determine the tidewater glacier status is the location of the calving front position and the separation of seasonal variability from long-term trends. Previous studies have proposed deep learning-based methods to semi-automatically delineate the calving fronts of tidewater glaciers. They used U-Net to segment the ice and non-ice regions and extracted the calving fronts in a post-processing step. In this work, we show a method to segment the glacier calving fronts from SAR images in an end-to-end fashion using Attention U-Net. The main objective is to investigate the attention mechanism in this application. Adding attention modules to the state-of-the-art U-Net network lets us analyze the learning process by extracting its attention maps. We use these maps as a tool to search for proper hyperparameters and loss functions in order to generate higher qualitative results. Our proposed attention U-Net performs comparably to the standard U-Net while providing additional insight into those regions on which the network learned to focus more. In the best case, the attention U-Net achieves a 1.5% better Dice score compared to the canonical U-Net with a glacier front line prediction certainty of up to 237.12 meters.

==> Glacier Calving Front SegmentationUsing Attention U-Net/00_abstract.tex <==
%One study subject of tidewater glaciers is their calving front position and their seasonal movement. Deep learning-based methods are exploited to semi-automatically delineate the calving fronts at Jakobshavn tidewater glacier. The state-of-the-art approach uses U-Net to segment the glacier and non-glacier regions and extracts the calving fronts in a post-processing step. 
An essential climate variable to determine the tidewater glacier status is the location of the calving front position and the separation of seasonal variability from long-term trends. Previous studies have proposed deep learning-based methods to semi-automatically delineate the calving fronts of tidewater glaciers. They used U-Net to segment the ice and non-ice regions and extracted the calving fronts in a post-processing step.
%
In this work, we show a method to segment the glacier calving fronts from SAR images in an end-to-end fashion using Attention U-Net. The main objective is to investigate the attention mechanism
%~\cite{AttUNet}
in this application. Adding attention modules to the state-of-the-art U-Net network %used in Zhang et al.~\cite{enze19}
lets us analyze the learning process by extracting its attention maps. We use these maps as a tool to search for proper hyperparameters and loss functions in order to generate higher qualitative results. Our proposed attention U-Net performs comparably to the standard U-Net while providing additional insight into those regions on which the network learned to focus more. In the best case, the attention U-Net achieves a \SI{1.5}{\percent} better Dice score compared to the canonical U-Net with a glacier front line prediction certainty of up to 237.12 meters.


==> Glacier Calving Front SegmentationUsing Attention U-Net/10_introduction.tex <==
\section{Introduction}\label{sec:introduction}
The Antarctic Peninsula is a hotspot of global warming. It has experienced a substantial temperature increase in the 20th century~\cite{absence}, strongly affecting its cryosphere. In 1995, the Prince-Gustav-Channel and Larsen-A ice shelves (floating extension of the glaciers) disintegrated~\cite{climatictrend}. The loss of ice shelves led to a reduction of the bracing forces on the tributary glaciers, which subsequently reacted by accelerating ice discharge and further retreat of the calving fronts~\cite{dynamicresponse,icedynamics,retreat}. The position of the calving front is an important variable to measure the glacier state. Its fluctuations can provide information about imbalances and a recession can destabilize the flow regime of an entire glacier system. Therefore monitoring the calving front positions is of high importance. 

Typically multi-spectral and synthetic aperture radar (SAR) remote-sensing imagery is used to map the position of the glacier calving fronts~\cite{remotesensing}. Manual delineation of the calving front position is applied in most studies, which is subjective, laborious, tedious and expensive~\cite{glacieraccuracy}. However, different (semi-)automatic routines using edge detection or image classification techniques were also developed. Baumhoer et al.~\cite{remotesensing} provide a detailed review on calving front detection approaches. Particularly in polar regions, the sea surface next to the calving front is often covered by the ice melange (sea ice and icebergs), making both the manual and automatic calving front detection challenging. 

Deep Convolutional Neural Networks (CNNs) have shown impressive performance in various image segmentation tasks. %DCNNs have the ability to detect small features and combine them with high-level feature maps. 
The first study using deep CNNs for calving front mapping on remote sensing imagery was conducted by Mohajerani et~al.~\cite{margins}. They applied the U-Net CNN architecture on Landsat imagery at glaciers in Greenland. Zhang et~al.~\cite{enze19} and Baumhoer et~al.~\cite{glacierextraction} applied similar processing pipeline on SAR imagery from either the TerraSAR-X or Sentinel-1 mission.
Today, there are many deep learning-based approaches and network architectures for image segmentation~\cite{DeepLearnSeg}. One of the most successful ones is the U-Net architecture%, developed in 2015 by Ronneberger et al.
~\cite{Unet}. 
%The combination of an autoencoder, convolutions, pooling layers, and skip connections aroused great interest. Therefore many approaches and versions of U-Net were developed. A new technology is coming up adding attention gates to the network. This architecture has been further improved by adding attention gates to the network {\color{red}{\cite{?}}}. Attention, in image classification, is a mechanism where salient regions of the image get highlighted in order to select a specific region of interest. This happens typically by applying a soft attention map to the image.
In 2018, Schlemper et~al.~\cite{Sononet} used soft attention gates in Sononet, which are able to localize salient regions in the feature maps. They introduced these gates to help the network preserve more local information and provide guided object localization in the forward pass. These gates use low-level features and global information gathered by the high-level feature maps in order to calculate an attention coefficient for each pixel. This approach was further enhanced by Oktay et~al.~\cite{AttUNet}. They added additive soft attention gates in the skip connections of the U-Net architecture. These gates learn the attention maps automatically without adding too much computational power. They are modular and can easily be implemented in the U-Net architecture. We use these gates together with the same U-Net model used in Zhang et~al.'s work~\cite{enze19} to detect the front positions on multi-mission SAR imagery. %Therefore, we select two glacier systems at the Antarctic Peninsula, which were former tributaries to the Larsen-A and Prince-Gustav-Channel ice shelves. 
Predicting thin fronts directly leads to a severe class-imbalance problem. %{\color{red}{We show different approaches and pre-processing methods to handle this problem. We extract the attention maps for each layer to see how well the network learns and where its attention is. We explain the concepts of distance weighted loss functions and how they can be used to generate qualitative good looking results. In the end, we show our qualitative and quantitative results of both networks regarding the choice of hyperparameters.}}
In this work, we extract the attention maps for each layer to see how well the network learns and where its attention is. Furthermore, we study the effect of distance weighted loss functions to alleviate this problem. 

% we could leave this out
%The rest of this paper is organized as follows: In Sec.~\ref{sec:methodology}, we introduce attention gates and present our workflow. Section~\ref{sec:experimental_setup} is dedicated to describe the dataset, to explain our experimental setup, and to present the quantitative and qualitative results. Finally, Sec.~\ref{sec:conclusion} concludes the paper.


==> Glacier Calving Front SegmentationUsing Attention U-Net/20_Methodology.tex <==
\section{Methodology}\label{sec:methodology}
~\\\noindent\textbf{Attention U-Net.}\noindent
\begin{figure*}[t]
%\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{Figures/Att-Unet.png}
	%\includegraphics[width=\linewidth]{Figures/Att-Unet.png}
	\caption{The architecture of our proposed Attention U-Net. }
	\label{fig:attunet}
\end{figure*}
%\end{figure}
%
%\subsection{Attention gates}\label{subsec:Attention_gate}
%Attention gates in U-Net firstly were proposed in the work ”Attention U-Net: Learning Where to Look for the Pancreas”\cite{AttUNet}. These gates 
Attention gates are modular building blocks, which can be placed into the skip
connections of a U-Net architecture~\cite{AttUNet}. We use a five-layered U-Net
model by Zhang et al.~\cite{enze19} as our base model, depicted in
\cref{fig:attunet}. %shows a $5$ layer Attention U-Net. %working on an input image of size $512 \times 512$ pixels. The input image gets convoluted, pooled and downscaled to $32 \times 32$ pixels. 
%
Each layer has two sequential blocks consisting of one two-dimensional convolution with a kernel size of $5 \times 5$ pixels and one batch normalization layer followed by a Leaky ReLU activation function. We use Max-Pooling to encode and shrink the feature maps on each layer and use transposed convolution in the upscaling path. 

We add attention gates to the same architecture and train and test it with the same data and hyperparameters.
Features (activation maps) $\bx^l$ %get extracted for each layer $l$ and 
are copied to the attention gates together with the gating signal $\bg^l$ taken
from the upscaling path. The number of feature maps $\fx$ of $\bx^l$ and $\fg$ of $\bg^l$ are reduced to $\fint$ intermediate layers by means of $1 \times 1$
convolution. Due to the coarser scale of the gating signal, the spatial
dimensions of $\bx^l$ are halved using strided convolution. To combine low-level
and high-level features maps, the intermediate layers are added and passed to a
ReLU activation function $\sigma_1$.
%Oktay et~al.~\cite{AttUNet} claim that %additive soft attention produces more accurate results than multiplicative attention. 
In order to obtain the attention coefficients, these layers are
combined through $\bm{\psi} \in \mathbb{R}^{\fint \times 1}$ (realized by a $1 \times
1$ convolution) and normalized by the Sigmoid
activation function $\sigma_2$, \ie for each pixel $i$ the attention coefficient
for layer $l$ follow as: 
%\Cref{eq:att_coef} shows the calculation of the attention coefficient for each pixel $i$:
%
\begin{equation}\label{eq:att_coef}
	\alpha^l_i =\sigma_2 (\bm{\psi}^T (\sigma_1 (\bW^T_x \bx^l_i + \bW^T_g \bg^l_i + \bb_g) + b_\psi) \enspace,
\end{equation}
%
where $\bW_x \in \mathbb{R}^{\fx \times \fint}$ and $\bW_g \in \mathbb{R}^{\fg \times \fint}$ are pixel-wise linear combinations of $\fx$ and $\fg$ feature maps and transformations to $\fint$ intermediate layers. The bias terms are denoted by $\bb_g \in \mathbb{R}^{\fint}$ and $b_\psi \in\mathbb{R}$. In the end, they are upscaled by a bilinear interpolation to the original spatial dimensions of the incoming feature maps. The attention coefficients $\alpha^l$ represent context-relevant regions. We apply the soft attention mechanism by pixel-wise multiplication of the attention maps and every feature map $x^l$, \ie: 
%
%\begin{equation}\label{eq:att_coef_mult}
	$\hat{x}^l_{i,c} = x^l_{i, c} \cdot \alpha^l_i$, % \enspace,
%\end{equation}
%
where $c$ describes the feature map index. %and $a^l_i$ denotes the attention coefficient for pixel $i$ in layer $l$. 
In this way, noisy and irrelevant regions in the feature maps get filtered out by the attention gate before going through the merging process. 
During training, those attention maps that localize the regions of interest are learned automatically.

%\subsection{Proposed workflow}
%An overview of our proposed workflow is shown in Fig.~\ref{fig:workflow}. 
In this work, we use Zhang et~al.'s U-Net architecture~\cite{enze19} as the baseline model in our semantic segmentation pipeline and add the attention gates to it, as depicted in \cref{fig:attunet}. %We use distance-weighted loss functions to tackle the severe class-imbalance. 
The attention gates narrow down the region of interest by automatically learning the glacier front line positions. Furthermore, the easily extractable attention maps demonstrate the learning quality evolution of the network.
%{\color{blue}{In the first we train Zhang et al.'s network~\cite{enze19} and the Attention U-Net on a dataset, which is splitted and pre-processed before. By means of distance weighted loss functions both models predict the front positions with specific uncertainties. Furthermore we extract the attention maps produced by the attention gates for each sample in the test set.}}
%

~\\\noindent\textbf{Distance-Weighted Loss Function.}\label{sec:dwloss}
\noindent
One big challenge in segmenting the front line directly is that a slight offset in the prediction heavily increases the loss. %The main goal of the networks is to predict the position and curvature of the calving glacier fronts. Predicting a thin line can lead to small deviations in position. 
%Therefore, we 
Adhikari et~al.~\cite{foresttrail} proposed to tolerate the network's
misprediction in a controlled close distance of the ground truth front line.
This is formulated and realized by calculating a weight map $\bW_w$:
\begin{equation}\label{eq:Ww}
	\bW_w = \sigma\left(\frac{\text{EDT}(\by)}{w}\right) \enspace,
\end{equation}
%
%coefficient for each
%pixel. 
which depends on the Euclidean distance transformation $\text{EDT}$ of the
ground truth map $\by$. Errors near the front line get weighted smaller than errors
further away. The weights are normalized by a Sigmoid function $\sigma$. With the parameter $w$, we can control the distance weighting. Bigger $w$
results in tolerance towards the mispredictions further away from the actual
front line. In this study, we explore weights $w =
\{4,8,16\}$. %\Cref{eq:Ww} expresses the weight map $\bW_w$:
%
%
%where $\text{EDT}(\by)$ describes the ground truth Euclidean-based distance transformation of the ground truth map $\by$.
The sigmoid output is zero-centered and added to the ground truth mask in order to omit weighting pixels within the glacier front, \ie:
%
%\begin{equation}
	$\widetilde{\bW}_w = 2(\bW_w - 0.5) + \by$. % \enspace.
%\end{equation}
%
The result of this transformation is shown in \cref{fig:dw_b}. This distance map contains the weighting coefficient for each pixel of the prediction $\hat{\by}$. We pixel-wise multiply the prediction and the distance-weighted map. The result is a distance-weighted prediction $\hat{\by}_w$, %, which is expressed in \cref{eq:yHat_w} and 
\cf \cref{fig:dw_d} for an example.
%
%\begin{equation}\label{eq:yHat_w}
%	\hat{y}_w = \widetilde{W}_w \cdot \hat{y}
%\end{equation}
%
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.20\linewidth}		
		\centering
		\centerline{\includegraphics[width=.87\linewidth]{Figures/gt_edt.png}}
		\caption{}\label{fig:dw_a}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.20\linewidth}		
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/weight_map.png}}
		\caption{}\label{fig:dw_b}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.20\linewidth}		
		\centering
		\centerline{\includegraphics[width=.87\linewidth]{Figures/pred_edt.png}}
		\caption{}\label{fig:dw_c}
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.20\linewidth}		
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/wpred.png}}
		\caption{}\label{fig:dw_d}
	\end{subfigure}
	%
	\caption{\subref{fig:dw_a} ground truth, \subref{fig:dw_b} weight map $\widetilde{\bW}_8$, \subref{fig:dw_c} prediction, and \subref{fig:dw_d} weighted prediction $\hat{\by}_8$.}
	\label{fig:distance_weighting}
\end{figure}
%
We use this modified prediction for the calculation of the BCE loss and non-binary Dice metric.
%, \ie: 
%
%\begin{equation}
%	\begin{aligned}
%		\text{WBCE}_w(\hat{y}, y) &= \text{BCE}(\hat{y}_w, y)\\
%		\text{WDice}_w(\hat{y}, y)&= \text{Dice}(\hat{y}_w, y)
%	\end{aligned}
%\end{equation}
%


==> Glacier Calving Front SegmentationUsing Attention U-Net/30_evaluation.tex <==
\section{Evaluation}\label{sec:experimental_setup}
%This section describes our dataset, pre-processing, and augmentation policies in our pipeline. Then we explain the network architecture, hyperparameters, and the concepts of distance-weighted loss functions. Finally, the qualitative and quantitative results will be presented.
\subsection{Dataset}\label{sec:dataset}
The SAR dataset is composed of imagery from the satellite missions ERS-1/2, Envisat, RadarSAT-1, ALOS, TerraSAR-X (TSX) and TanDEM-X (TDX). It contains $244$ images showing the glacier systems of Sjögren-Inlet (SI) and Dinsmoore-Bombardier-Edgworth (DBE) located in the Antarctic Pensula. Together, they cover the time period of 1995-2014. We use multilooking to reduce speckle in the image and take the refined ASTER digital elevation model~\cite{cook2012new}  of the Antarctic Peninsula for geocoding and orthorectification. 
%
\begin{comment}
More detailed parameters of the SAR sensors and imagery are shown in Tab.~\ref{tab:sar_sensors}. 
%
\begin{table}[htbp]
	\centering
	\setlength{\tabcolsep}{3pt}
	\begin{tabular}{c|c|c|c|c|c}

		\hline
		Platform & Sensor & Mode & \makecell{Repetition\\ cycle [d]} & \makecell{Multi \\ looking\\ factors} & \makecell{Ground \\range\\ %resolution [m]}\\ \hline
		ERS-1/2 & SAR & IM & 53/1 & $1\times5$ & 20 \\\hline
		\makecell{RADARSAT 1 \\ (SLC+PRI) }& SAR & ST & 24 & $1\times4$ & \makecell{20 (SLC) \\ 12.5 (PRI)} \\  \hline
		Envisat & ASAR & IM & 35 & $2\times5$ & 20 \\ \hline
		ALOS & PAlSAR & FBS & 46 & $2\times5$& 16.7 \\ \hline 
		\makecell{TerraSAR-X \\ tanDEM-X \\ (SLC format)} &SAR & SM & 11 & $3\times 3$ & 6.7 \\ \hline
	\end{tabular}
	\caption{Overview of SAR sensors and specifications used in this study.}
	\label{tab:sar_sensors}
\end{table}
\end{comment}
%
We split this dataset into $144$ samples for training, $50$ for validation and $50$ for testing. As for the expert data annotation, we exploited the front positions used by Seehaus et al.~\cite{icedynamics, dynamicresponse}. 
\begin{comment}
They manually localized and picked the fronts with different qualities. Due to the similarity of the glacier and the ice melange, the accuracy of their manual front detection varies between 70 meters and 450 meters. On average, there is an uncertainty of $\approx$ \SI{200}{m}.
\end{comment}
%
\begin{figure}[t]
	\centering
	\mbox{%
	\includegraphics[width=\linewidth]{Figures/predictions_small.jpg}
	\phantomsubcaption\label{fig:p_a}	\phantomsubcaption\label{fig:p_b}	\phantomsubcaption\label{fig:p_c}	\phantomsubcaption\label{fig:p_d}
	}%
	\caption{Predictions of both networks trained on different weights for two samples of the test set. \subref{fig:p_a} and \subref{fig:p_c} are predicted by the U-Net approach~\cite{enze19}, and \subref{fig:p_b} and \subref{fig:p_d} show the results produced by our Attention U-Net; green: ground truth, red: prediction, yellow: intersection of the ground truth and the prediction.}
	\label{fig:predictions}
\end{figure}
%
\subsection{Evaluation Protocol}
%\subsubsection{Pre-processing}\label{sec:preprocess}
%Since different sensors are used for the imagery, the SAR images are captured with different resolutions. Thus, pixel information density differs for each sample in our dataset. We use median filtering with a filter size based on the pixel resolution of the sensor. Instead of filtering with a fixed pixel-based kernel size, we adapt our median filter to filter a region of \SI{2500}{m^2}. The resulting discrete kernel size is rounded up to the nearest uneven integer. That is, for a SAR image with a pixel width of \SI{20}{m}, a kernel size of $3\times3$ pixels is used. This step filters out high-frequency noise and helps to prevent aliasing effects in the downscaling process. Next, we applied zero-padding on the images to form squares and then resized the images to $512 \times 512$ pixels with bilinear interpolation. At this point, the average spatial resolution of the downscaled dataset is \SI{2001.84}{m^2}. For the pre-processing of the corresponding glacier fronts, the first step is to thicken our lines in the ground truth with a morphological operator. Since the purpose of the networks is to segment these lines directly, we consequently have a big class imbalance, which is about 2000:1 without pre-processing. This means that for each pixel located in the front, 2000 other pixels belong to the background. Without thickening, the networks would predict mostly a black image and front localization would fail due to the class imbalance. Thus, we use a dilation operator on the ground truth mask so that after the downscaling the fronts are 6 pixels thick. This implies that the networks are forced to predict thicker lines so that we add an uncertainty of six pixels to the prediction. However, this improves the class ratio of the background to the fronts to 100:1. We use two different kinds of data augmentation. The combination of four 90 degree rotations with flips increases our training and validation dataset by eight times.
We applied median filtering for noise reduction. Since the images in the dataset have different spatial resolutions, we used an adaptive kernel size, such that it covers a region of \SI{2500}{m^2}. Next, we applied zero-padding on the images to form squares and then resized the images to $512 \times 512$ pixels using bilinear interpolation. In order to alleviate the severe class-imbalance problem, we used morphological dilation to thicken the glacier front lines in the ground truth images such that they became $6$ pixels wide after downscaling. This reduces the class-imbalance severity from approximately 2000:1 to 100:1. Additionally, we augmented our training set using vertical flips and rotated versions ($90^\circ$, $180^\circ$ and $270^\circ$).

%\subsubsection{Network Architecture and Hyperparameters}
%We use the U-Net model by Zhang et al.~\cite{enze19} as our base model. %Despite the fact that his team uses this network for patch-wise image segmentation, we are using the same model for the line segmentation of glacier fronts in SAR images, which are resized to $512 \times 512$ pixels. 
%The network consists of five layers. 
%In the U-Net, each layer produces feature maps $x^l$, which are copied to skip connections and get merged with feature maps from the upscaling path. In the end, all feature maps get combined to one image on which the Sigmoid activation function gets applied. 
%To understand the learning process of this network, we add attention gates to the same architecture and train and test it with the same data and hyperparameters. \Cref{fig:attunet} depicts the structure of our proposed Attention U-Net. 
%In the first four layers, feature maps $x^l$ are fit into these gates together with a gating signal $g^l$ taken from the upscaling path. To increase the capacity of the gating coefficient, we double the feature maps of the gating signal by $1\times1$ convolutions followed by a Batch Normalization layer and a ReLU activation function. The attention gates weight incoming features maps with attention maps $\alpha^l$, which results in a weak object localization in the forward pass. %Section~\ref{sec:methodology} explains this process in more details.
For training the networks, we used Adaptive Moment Estimation (ADAM) optimizer
with a batch size of $5$ and a cyclic learning rate with minimum and maximum boundaries of $10^{-5}$ and $10^{-3}$, respectively. 
% let's leave that out, actually the ReLU/LeakyReLU activation functions
% should have initialized by He initialization 
%We used Xavier weight initialization. 
For the Leaky ReLU activation functions, we set the slope to $0.1$. 
As for the loss function, we used the normal Binary Cross-Entropy (BCE) in one variant
and the distance-weighted BCE (WBCE) in the other variant. We monitored the Dice coefficient and its modified version for early stopping with a patience of $20$ epochs. 
%The U-Net architecture has about 24M trainable parameters. By adding attention gates, we increase this number by 400000. Therefore, not much additional computational power is needed to train the Attention U-Net.

%\subsection{Qualitative and Quantitative Results}
%We first show the qualitative results of both networks with different weight parameters. In addition, we analyze the attention maps produced by the attention gates. Then, we present our quantitative results and compare them with the state-of-the-art (SOTA) results by Zhang et~al.~\cite{enze19}.

\subsection{Qualitative Results} \label{sec:qualitativ}
\Cref{fig:predictions} illustrates the predictions of two glacier fronts using U-Net and Attention U-Net, trained on a distance-weighted BCE loss with different weights. %We generate the binary predictions based on a specific boundary $t$, which is explained in Sec.~\ref{sec:quantitativ}. 
%The green color indicates the ground truth, red shows the prediction, and the yellow line is the intersection of the ground truth and the prediction. 
It shows that our proposed Attention U-Net outperforms U-net for big distance weights, especially for $w=16$, as shown in \cref{fig:predictions}. %Training on a distance-weighted loss function leads to predictions with different uncertainty. 
Note, increasing $w$ results in thicker predicted lines and consequently higher uncertainty. 
%
\begin{comment}
\begin{figure}[tbp]
	\centering
	\includegraphics[width=.75\linewidth]{Figures/thickness.png}
	\caption{Predictions of U-Net trained on BCE loss with weights: (a) no weighting, (b) $w=4$, (c) $w=8$, and (d) $w=16$.}
	\label{fig:thickness}
\end{figure}
\end{comment}
%
Using the normal BCE loss often results in disconnected predicted lines. While WBCE mitigates this problem, this can sometimes be a disadvantage, \eg when mountains near the front lines  cause gaps on the ground truth line due to layover and shadowing. \Cref{fig:p_a} and \cref{fig:p_b} show that networks trained on weight parameter greater than four fail to localize small gaps and simply connect the predicted fronts. %As a result, training on a distance-weighted loss function has its positive and negative effects.
%Focusing on Fig.~\ref{fig:predictions}-c and Fig.~\ref{fig:predictions}-d, both models trained using $WBCE_{16}$ show inaccuracies in predicting the correct position and curvature. Since false positive predictions get less punished for a high weight parameter, the models tend to predict fronts with different shapes. 
%However, \cref{figp_c} depicts that the standard U-Net produces artifacts, such as circles near the fronts for WBCE$_16$, while the Attention U-Net produces more accurate predictions.

We can analyze the learning process of Attention U-Net by means of the attention maps $\alpha^l$, extracted from layer $l$. 
%Since this network architecture consists of four attention gates, we get four attention maps with different dimensions: $\alpha^1: 512\times512$ pixels, $\alpha^2: 256\times256$ pixels, $\alpha^3: 128\times128$ pixels, and $\alpha^4: 64\times64$ pixels. 
\Cref{fig:attention_2007_1_1} shows the evolution of the attention maps (resized to the same scale). 
%
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{Figures/attention_maps_2007_1_1_cut.png}
	\caption{Attention maps $\alpha^l$ for models saved at epoch 5, 10, and 36.}
	\label{fig:attention_2007_1_1}
\end{figure}
%
We observe that the attention maps converge quickly within the first epochs to the regions of interest. In general, attention maps $\alpha^4$ and $\alpha^3$ look more noisy than $\alpha^2$ and $\alpha^1$. However, this shows that the attention gates can learn salient regions automatically, even in the bottom layers of a U-Net. 
Besides the glacier front, there is also a weak highlighting on the zero-padded border and other regions like mountains and ice melange located near the front. This may help the network to recognize specific glacier systems. 

\Cref{fig:attention_maps_weights} shows the effect of different distance weights on the attention maps. Training on a distance-weighted loss function with a small weight reduces noisy highlights in the attention maps, especially in layer $3$. When increasing the weight too much, the attention gates cannot localize the regions of interest in the low-level feature maps, as shown in \cref{fig:a_d}. 
%The predictions and their corresponding attention maps illustrate that a too big weight $w$ results in qualitative worse outcomes.
Choosing a weight between $w=4$ and $w=8$ lead to the best qualitative results in our test set.
%
\begin{figure}[t]
	\centering
	\mbox{%
	\includegraphics[width=.6\linewidth]{Figures/attention_maps_weights.png}
	\phantomsubcaption\label{fig:a_a}	\phantomsubcaption\label{fig:a_b}	\phantomsubcaption\label{fig:a_c}	\phantomsubcaption\label{fig:a_d}
}%
\caption{Attention maps for models trained on \subref{fig:a_a} BCE, \subref{fig:a_b} $\mathrm{WBCE}_4$, \subref{fig:a_c} $\mathrm{WBCE}_8$, and \subref{fig:a_d} $\mathrm{WBCE}_{16}$.}
	\label{fig:attention_maps_weights}
\end{figure}

\subsection{Quantitative Results}\label{sec:quantitativ}
\begin{table}[t]
	\centering
	%\normalsize
	\caption{Quantitative results of the U-Net, with and without the attention
		gates.%
		%measured with distance-weighted Dice coefficients ($\mathrm{WDice}_{w}$) and Intersection over Union (IoU).
}
	\small
	\begin{tabular}{@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }}
		\toprule
		Model & Loss & Dice & $\mathrm{WDice}_4$ & $\mathrm{WDice}_8$&
		$\mathrm{WDice}_{16}$ & IoU \\ 
		\midrule
		U-Net & BCE &\h{73.9} & \h{83.0} & \h{86.0} & 88.3 & \h{60.6} \\
			Att. U-Net & BCE &73.8 & 82.9 & 85.9 & \h{88.7} & 60.3 \\
		\midrule
		U-Net & $\mathrm{WBCE}_4$ &\h{72.9} & \h{83.6} & \h{87.1} & \h{90.1} & \h{58.9} \\
		Att. U-Net & $\mathrm{WBCE}_4$ &72.6 & \h{83.6} & 87.0 & 89.9 & 58.5 \\
		\midrule
		U-Net & $\mathrm{WBCE}_8$ &70.1 & 81.1 & 84.6 & 87.6 & 55.5 \\
		Att. U-Net & $\mathrm{WBCE}_8$ &\h{70.8} & \h{82.5} & \h{86.1} & \h{89.2} & \h{56.1} \\
		\midrule
		U-Net & $\mathrm{WBCE}_{16}$ &\h{67.0} & \h{78.9} & \h{82.6} & 85.9 & \h{51.9} \\    
		Att. U-Net & $\mathrm{WBCE}_{16}$ &65.2 & 77.8 & 82.3 & \h{86.1} & 49.8 \\ 
		\bottomrule
	\end{tabular}
	\label{tab:quantitativ}
\end{table}

\Cref{tab:quantitativ} presents quantitative results for our test set. 
%It shows the average thickness of the predicted front lines, produced by WBCE with different weights, in pixels and the corresponding uncertainty in meters. %We convert the predictions to binary predictions based on a binary decision boundary $t$. We classify prediction values above $t$ as a one and values below the threshold as zero. We scan for the best boundary with a step size of 0.01 for each metric. In most of our runs, this boundary is between 0.1 and 0.5. 
Overall, the results show that Attention U-Net performs similar to the base U-Net with the advantage of better interpretability. In case of a distance weight of 8 (WBCE$_8$), Attention U-Net performs significantly better than the base model. Distance-weighted Dice scores with bigger weights are generally better since errors near the front are weighted smaller.
%
%
\begin{table}[t]
	\centering
	%\normalsize
	\caption{Average thickness of the predicted lines in pixels and the resulting certainty (perpendicular to the estimated glacier front position) based on an average spatial resolution of \SI{44.74}{m}.}
	\small
	\begin{tabular}{cccccc}
		\toprule
		$w$ & 0 & 4 & 8&16 \\ 
		\midrule
		thickness [px] & 6.5 & 8.4 & 10.6 &  11.1  \\ 
	  certainty [m]  & 145.40 & 187.90 & 237.12 & 248.30 \\ 
		\bottomrule
	\end{tabular}
	\label{tab:uncertainty}
\end{table}
%
Assuming a small amount of misprediction, we can estimate the average thickness of the lines by the class ratio of front to the background. \Cref{tab:uncertainty} shows that training on BCE with different weights leads to front predictions with different thicknesses and certainties.
%
\begin{comment}
\begin{table}[htbp]
	\centering
	%\normalsize
	\small
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		$w$ & 0 & 4 & 8&16 \\ \hline
		\makecell{thickness\\ $[$px$]$} & 6.5 & 8.4 & 10.6 &  11.1  \\ \hline
		\makecell{certainty \\ $[$m$]$} & 145.40 & 187.90 & 237.12 & 248.30 \\ \hline
	\end{tabular}
	\caption{Average thickness of the predicted lines in pixels and the resulting certainty $($perpendicular to estimated glacier front position$)$ based on an average pixel resolution of \SI{44.74}{m}.}
	\label{tab:uncertainty}
\end{table}
%
Although, the loss scales nearly linearly to the weight and the distance, the thickness of the predicted lines does not. Doubling $w$ does not mean that the lines are getting two times thicker. However, increasing the weight too much leads to a significant performance decrease, which also can be observed in the qualitative results, as explained in Sec.~\ref{sec:qualitativ}. 
\end{comment}
%
With $w=4$, we obtain a Dice score of \SI{83.6}{\percent} with a tolerance of $187.90$ meters. It is possible to reduce this uncertainty by using a smaller dilation kernel, smaller distance weight, or a patch-wise line segmentation with a higher pixel resolution.

%Zhang et al.~\cite{enze19} proposed a different approach to predict glacier front positions. They use a patch-wise image segmentation to predict ice melange regions and consequently extract the glacier front lines through region separation in a post-processing step. Dividing the image into small patches of size $960 \times 720$ pixels leads to a more precise pixel resolution of \SI{6}{m}. Apart from the manual delineation errors, they obtain an average accuracy of $38$ meters ($\sim$ $6$ pixels). In terms of certainty, their patch-wise method shows better results. However, multiple forward passes and an additional post-processing step are needed to generate one prediction 


==> Glacier Calving Front SegmentationUsing Attention U-Net/40_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In summary, this study shows that it is possible to delineate calving glacier fronts by means of a trained U-Net in a single forward pass without additional post-processing. The addition of attention gates revealed insights into the learning behavior of the network. Within a few epochs, the network learns to localize important regions automatically and shows where its attention is. Our results show that the attention mechanism itself improves our predictions for big distance weights. Furthermore, it can be used as an analysis tool to find proper loss functions and hyperparameters. Consequently, we conclude that training on a distance weighted version of Binary Cross-Entropy with a small weight parameter leads to optimal qualitative and quantitative results.

